Event-Based Crossing Dataset (EBCD)

Event-based vision revolutionizes traditional image sensing by capturing asynchronous intensity variations rather than static frames, enabling ultrafast temporal resolution, sparse data encoding, and enhanced motion perception. While this paradigm offers significant advantages, conventional event-based datasets impose a fixed thresholding constraint to determine pixel activations, severely limiting adaptability to real-world environmental fluctuations. Lower thresholds retain finer details but introduce pervasive noise, whereas higher thresholds suppress extraneous activations at the expense of crucial object information. To mitigate these constraints, we introduce the Event-Based Crossing Dataset (EBCD), a comprehensive dataset tailored for pedestrian and vehicle detection in dynamic outdoor environments, incorporating a multi-thresholding framework to refine event representations. By capturing event-based images at ten distinct threshold levels (4, 8, 12, 16, 20, 30, 40, 50, 60, and 75), this dataset facilitates an extensive assessment of object detection performance under varying conditions of sparsity and noise suppression. We benchmark state-of-the-art detection architectures-including YOLOv4, YOLOv7, EfficientDet-b0, MobileNet-v1, and Histogram of Oriented Gradients (HOG)-to experiment upon the nuanced impact of threshold selection on detection performance. By offering a systematic approach to threshold variation, we foresee that EBCD fosters a more adaptive evaluation of event-based object detection, aligning diverse neuromorphic vision with real-world scene dynamics. We present the dataset as publicly available to propel further advancements in low-latency, high-fidelity neuromorphic imaging: https://ieee-dataport.org/documents/event-based-crossing-dataset-ebcd

==> conclusion.tex <==
\section*{Conclusion}
\label{sec:conclusion}
Conventional high-resolution imaging suffers from energy and bandwidth issues due to the back-and-forth frame-by-frame data transfer of sensor and neural networks. Event sensors reduce these bottlenecks by introducing event-vision. However, the need for open-source event data, in particular, human face data with annotations, is one of the major bottlenecks in event-vision research. Besides, generating event data for faces is a challenging task. In this paper, we overcome this event data issue by proposing a programmable, digital threshold-based event dataset considering four thresholds (i.e., 4, 8, 12, and 16). 

In addition to the thresholded datasets, a threshold-based smart event generation algorithm was presented to generate desired
thresholded datasets. The tool flow will enable more research in event-vision. %In this paper, we also discussed the existing neural architectures for object detection and localization. 
We verified the effectiveness of our data using existing YOLO-v4, EfficientDet-b0, and MobileNets-v1 object detection and localization models. All three architectures achieve excellent AP50, 95.05\%, 98.08\%, and 96.69\% for YOLO-v4, EfficientDet-b0, and MobileNets-v1, respectively using the same threshold
= 8 valued dataset.
\vspace{-0.60cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Dummy%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



